Liquid-activated quantum emission from pristine hexagonal boron nitride for nanofluidic sensing

Liquids confined down to the atomic scale can show radically new properties. However, only indirect and ensemble measurements operate in such extreme confinement, calling for novel optical approaches enabling direct imaging at the molecular level. Here, we harness fluorescence originating from single-photon emitters at the surface of hexagonal boron nitride (hBN) for molecular imaging and sensing in nanometrically confined liquids. The emission originates from the chemisorption of organic solvent molecules onto native surface defects, revealing single-molecule dynamics at the interface through spatially correlated activation of neighboring defects. Emitter spectra further offer a direct readout of local dielectric properties, unveiling increasing dielectric order under nanometer-scale confinement. Liquid-activated native hBN defects bridge the gap between solid-state nanophotonics and nanofluidics, opening new avenues for nanoscale sensing and optofluidics.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
